Magnetic Fields in Massive Star-Forming Regions (MagMaR) II. Tomography Through Dust and Molecular Line Polarization in NGC 6334I(N)

Here, we report ALMA detections of polarized emission from dust, CS($J=5 \rightarrow 4$), and C$^{33}$S($J=5 \rightarrow 4$) toward the high-mass star-forming region NGC6334I(N). A clear ``hourglass'' magnetic field morphology was inferred from the polarized dust emission which is also directly seen from the polarized CS emission across velocity, where the polarization appears to be parallel to the field. By considering previous findings, the field retains a pinched shape which can be traced to clump length-scales from the envelope scales traced by ALMA, suggesting that the field is dynamically important across multiple length-scales in this region. The CS total intensity emission is found to be optically thick ($\tau_{\mathrm{CS}} = 32 \pm 12$) while the C$^{33}$S emission appears to be optically thin ($\tau_{\mathrm{C^{33}S}} = 0.1 \pm 0.01$). This suggests that sources of anisotropy other than large velocity gradients, i.e. anisotropies in the radiation field are required to explain the polarized emission from CS seen by ALMA. By using four variants of the Davis-Chandrasekhar-Fermi technique and the angle dispersion function methods (ADF), we obtain an average of estimates for the magnetic field strength onto the plane of the sky of $\left< \mathrm{B}_{\mathrm{pos}} \right> = 16$ mG from the dust and $\left< \mathrm{B}_{\mathrm{pos}} \right> \sim 2$ mG from the CS emission, where each emission traces different molecular hydrogen number densities. This effectively enables a tomographic view of the magnetic field within a single ALMA observation.

==> ms_header.tex <==

%%%%%%%%%%%%%%
% Short cuts %
%%%%%%%%%%%%%%

% Astrometry Units

\newcommand{\hr}{\mbox{$^h$}}
\renewcommand{\min}{\mbox{$^m$}}
\renewcommand{\sec}{\mbox{$^s$}}
\renewcommand{\deg}{\mbox{$^{\circ}$}}
%\newcommand{\arcmin}{\mbox{$^'$}}
%\newcommand{\arcsec}{\mbox{$^{''}$}}
\newcommand{\kms}{\mbox{km\,s$^{-1}$}}
\newcommand{\fluxunits}{\mbox{erg\,cm$^{-2}$ s$^{-1}$}}
\newcommand{\uJy}{\mbox{$\mu$Jy}}
\newcommand{\um}{\mbox{$\mu$m}}
\newcommand{\ULL}{\mbox{$<27.0$}}
% Miscellaneous
\newcommand{\dbrk}{\mbox{$D(4000)$}}
\newcommand{\wrst}{\mbox{$W_{\lambda}^{\mbox{\tiny rest}}$}}
\newcommand{\wrsti}{\mbox{$W_{\lambda,i}^{\mbox{\tiny rest}}$}}
\newcommand{\wobs}{\mbox{$W_{\lambda}^{\mbox{\tiny obs}}$}}
\newcommand{\haln}{\mbox{H$\alpha$(n)}}
\newcommand{\halb}{\mbox{H$\alpha$(b)}}
\newcommand{\simgtr}{\, \raisebox{-.2ex}{$\stackrel{>}{\mbox{\tiny $\sim$}}$} \,}
\newcommand{\simlt}{\, \raisebox{-.2ex}{$\stackrel{<}{\mbox{\tiny $\sim$}}$} \,}
\newcommand{\sigsky}{\mbox{$\sigma_{\mbox{\tiny sky}}$}}
\newcommand{\bootes}{Bo\"{o}tes}
\newcommand{\lamfwhm}{\mbox{$\Delta \lambda_{\mbox{\tiny FWHM}}$}}
\newcommand{\lamblaze}{\mbox{$\lambda_{\mbox{\tiny blaze}}$}}
\newcommand{\rarrow}{\mbox{$\Rightarrow$}}
\newcommand{\fshrt}{\mbox{$f_{\tiny \nu}^{\mbox{\tiny short}}$}}
\newcommand{\flng}{\mbox{$f_{\tiny \nu}^{\mbox{\tiny long}}$}}
\newcommand{\ztit}{\mbox{$z \approx 4.5$}}
\newcommand{\x}{\mbox{$\times$}}
\newcommand{\Msun}{\mbox{M$_{\odot}$}}
\newcommand{\Mdot}{\mbox{$\dot{m}_{-4}$}}
\newcommand{\Lsun}{\mbox{L$_{\odot}$}}
\newcommand{\E}[1]{\hbox{$10^{ #1 }$}}
\newcommand{\per}[1]{\hbox{#1$^{-1}$}}
\newcommand{\tothe}[1]{\hbox{$^{#1}$}}
\newcommand{\about}{\mbox{$\sim$}}
\newcommand{\SIG}{\mbox{W~m$^{-2}$~Hz$^{-1}$~sr$^{-1}$}}
\newcommand{\nISM}{\mbox{$n_{\rm ISM}$}}
%\newcommand{\uJy}{\mbox{$\mu$Jy}}
%\newcommand{\about}{\mbox{$\sim$}}
\def\IRAS       {\hbox{\it IRAS}}
\def\NVSS       {\hbox{\it NVSS}}

\def\OIII       {\hbox{O\tiny{III}}}
\def\NII        {\hbox{N\tiny{II}}}
\def\NO         {\hbox{---}}
\def\HII        {\hbox{H \small{II}}}
\def\Htwo       {\hbox{H_{2}}}
\def\HI         {\hbox{H \small{I}}}
\def\Ha         {\hbox{H \small{$\alpha$}}}
\def\Hb         {\hbox{H \small{$\beta$}}}
\def\SFIR       {\hbox{$S_{\rm FIR}$}}
\def\HCOP       {\hbox{HCO$^{+}$}}
\def\thirCO     {\hbox{$^{13}$CO}}
\def\water      {\hbox{H$_{2}$O}}
\def\source     {\hbox{G30.79\,FIR\,10}}

